Implicit-Explicit Time Integration for the Immersed Wave Equation

Immersed boundary methods simplify mesh generation by embedding the domain of interest into an extended domain that is easy to mesh, introducing the challenge of dealing with cells that intersect the domain boundary. Combined with explicit time integration schemes, the finite cell method introduces a lower bound for the critical time step size. Explicit transient analyses commonly use the spectral element method due to its natural way of obtaining diagonal mass matrices through nodal lumping. Its combination with the finite cell method is called the spectral cell method. Unfortunately, a direct application of nodal lumping in the spectral cell method is impossible due to the special quadrature necessary to treat the discontinuous integrand inside the cut cells. We analyze an implicit-explicit (IMEX) time integration method to exploit the advantages of the nodal lumping scheme for uncut cells on one side and the unconditional stability of implicit time integration schemes for cut cells on the other. In this hybrid, immersed Newmark IMEX approach, we use explicit second-order central differences to integrate the uncut degrees of freedom that lead to a diagonal block in the mass matrix and an implicit trapezoidal Newmark method to integrate the remaining degrees of freedom (those supported by at least one cut cell). The immersed Newmark IMEX approach preserves the high-order convergence rates and the geometric flexibility of the finite cell method. We analyze a simple system of spring-coupled masses to highlight some of the essential characteristics of Newmark IMEX time integration. We then solve the scalar wave equation on two- and three-dimensional examples with significant geometric complexity to show that our approach is more efficient than state-of-the-art time integration schemes when comparing accuracy and runtime.

==> content/brainstorming.tex <==

A short summary of application fields of IMEX methods.
\begin{itemize}
    \item first introduction by Belytschko and Mullen in \cite{BM78} in the context of structural mechanics (stability investigation, original 1976 not  found)
    \item Hughes et al avoiding interface elements \cite{H78, H78_stability}. Nicoli et al also \cite{HPL79} (Newmark based with parameters still variable, pseudo static system)
    \item Runge-Kutta- or Runge-Kutta-Nyström- based:
    chemistry (diffusion reaction) \cite{SSV05}, weather simulation \cite{WLW13, R18}, ... (noch weiter übertragen)
    
    \item For application to Cahn-Hillard flow \cite{R18} (Also cfd, phillips Paper)
    \item \cite{A95} convection diffusion
    \item imex generalized alpha \cite{MFH89}
    \item \cite{Extrapolation2010}
    \item for fractional differential equations https://www.sciencedirect.com/science/article/abs/pii/S0168927420301215
    
    \item sheet metal forming \cite{sheatMetal}, interessante Citations aus dem Multibody bereich
    
    \item Discontinuous Galerkin IMex Runge Kutta https://www.sciencedirect.com/science/article/abs/pii/S0010465509001490, combined as FSI https://www.sciencedirect.com/science/article/abs/pii/S0021999114002216
    \item for multiphysical modeling of layered structures (auch Runge Kutta Imex) \cite{CT11}
    \item hydrodynamics, nonlinear heat conduction https://www.sciencedirect.com/science/article/abs/pii/S0021999110000069
    \item boundary element method, kein Fulltext findbar...
    
    \item "implicit-explicit time integration, immersed" (google scholar)
    \item In the literature, RK Imex approaches are common. However, in the context of wave propagation cdm is very popular (belegen), hence why an Newmark IMEX is an obvious choice.
    
\end{itemize}


Struktur Paper:

Introduction
    Motivation aus MA 
    
Spatial Discretization
    Motivation und Basics für SCM (ähnlich wie MA, nur kürzer)
    
Time Integration
    Central Difference Method (hier auch auf auf Lumping eingehen?)
    Implicit methods
    IMEX methods (siehe MA, algemein, dann Newmark IMEX darstellen)
    
Benchmark Setups (nach setups/results vs nach beispiel gliedern?)
    Plate with Hole
    some larger 3D one
    
Results
    forward simulation
    convergence plots
    
Conclusions
    Vermerk zu FWI (hierbei auch adaptive implicit/Explicit subgroups erwähnen? falls ja ähnlich zu Soares) 
    
    
    
